Grounding Hierarchical Vision-Language-Action Models Through Explicit Language-Action Alignment

Achieving robot transparency is a critical step toward effective human-robot collaboration. To be transparent, a robot's natural language communication must be consistent with its actions and explicitly grounded in the task and environment. Existing hierarchical Vision-Language-Action (VLA) models can generate language (e.g., through chain-of-thought) and low-level actions. However, current work does not consider explicit alignment between these modalities during training. To address this crucial gap, we propose a novel training framework that explicitly grounds hierarchical VLA sub-task descriptions with respect to the visual observation and action space. Our framework uses a contrastive model to assess the alignment between generated language and corresponding action trajectories. This contrastive model enables direct ranking of different language-trajectory pairs based on their alignment, allowing us to refine the grounding of our hierarchical VLA through offline preference learning. We apply our framework to the LanguageTable dataset, a benchmark dataset of human language-annotated trajectories, and provide critical insights into multimodal grounding representations, all while establishing a strong baseline that achieves performance comparable to fully supervised fine-tuning and minimizing the need for costly data annotations.

==> abstract.tex <==
% \begin{abstract}
% Achieving robot transparency is a critical step toward human-robot collaboration.
% To be transparent, a robot's natural language explanations must be consistent with its actions and grounded in the task and environment.
% While existing Vision-Language-Action (VLA) models can generate language (e.g., through chain-of-thought) and decode low-level actions, they lack a mechanism to explicitly align and evaluate the consistency between the two.
% We propose a novel framework that extends VLA models to create an action-language grounded transparent agent, capable of generating both human-understandable utterances and corresponding action trajectories. 
% Our framework uses a contrastive model to explicitly evaluate the alignment between generated language and action trajectories.
% Furthermore, the contrastive model allows us to directly rank different language-trajectory pairs based on their alignment, enabling us to use offline preference learning to refine our transparent VLA's grounding.
% We demonstrate the effectiveness of our approach on the LanguageTable dataset, showing improvements in language-action consistency and task following.
% \end{abstract}
